Shift Invariance Can Reduce Adversarial Robustness

Shift invariance is a critical property of CNNs that improves performance on classification. However, we show that invariance to circular shifts can also lead to greater sensitivity to adversarial attacks. We first characterize the margin between classes when a shift-invariant linear classifier is used. We show that the margin can only depend on the DC component of the signals. Then, using results about infinitely wide networks, we show that in some simple cases, fully connected and shift-invariant neural networks produce linear decision boundaries. Using this, we prove that shift invariance in neural networks produces adversarial examples for the simple case of two classes, each consisting of a single image with a black or white dot on a gray background. This is more than a curiosity; we show empirically that with real datasets and realistic architectures, shift invariance reduces adversarial robustness. Finally, we describe initial experiments using synthetic data to probe the source of this connection.

==> sections/MaterialWeWontUse.tex <==

\subsection{Adversarial Examples in Linear Regression}

We first consider the way in which adversarial examples can occur in linear regression.  We consider regression based on a two-class classification problem, in which all points have a label of 1 or -1.  We show that when there are a large number of training points in a very high-dimensional space, in which most features are noisy and irrelevant, adversarial examples will occur.  This is somewhat surprising, because linear regression is so simple.

Let $x_i \in {\cal R}^d, i = 1, ... n$ be a set of training points.  Let $y_i \in \{-1,1\}$ denote the label of $x_i$.  We denote $X = \{x_i\}, Y = \{y_i\}$.

We now consider the following simple regression problem.  Suppose the $x_i$ are i.i.d.~from a Gaussian distribution with zero mean and variance $\sigma$.  Let $x_i(1)$ denote the first coordinate of $x_i$.  Let $y_i = sign(x_i(1))$.  That is, the label of $x_i$ depends only on its first coordinate; all other coordinates are irrelevant.  We also assume that $n << d$ and that $\sigma = \frac{1}{\sqrt{d}}$ (this last assumption isn't really important, but may be convenient, because $E(\|x_i\|) = 1$).  Let $f^*$ denote a function that fits the data perfectly, that is, $f^*(x_i) = y_i$.  In this section we will only consider the case in which $f^*$ is linear.

We can define $f^*$ using a vector $w$, in which $f^*(x_i) = w^Tx_i$.  Note that for any choice of $X$ and $Y$ there will be many possible choices of $f^*$.  To see this, let $\cal X$ denote the linear subspace spanned by $X$, and let ${\cal X}^\perp$ denote linear subspace orthogonal to $\cal X$.  Then any component of $w$ that lies in ${\cal X}^\perp$ is irrelevant to the value $f^*(x_i)$.  We will assume that all such components of $w$ are equal to zero, so that $w \in \cal X$.  

It is easy to see that in fact $w \in {\cal X}$ if we compute $w$ using gradient descent, after initializing $w \in {\cal X}$.  {\em Fill in this proof}

\sg{Let $\mathcal{L}$ be any first order differentiable loss function, then the update step gradient is $\mathbf{w}^{(t+1)}=\mathbf{w}^{(t)}-\eta_{t} \nabla_{\mathbf{w}} \mathcal{L}(\mathbf{w}) = \mathbf{w}^{(t)}-\eta_{t} \nabla_{f} \mathcal{L}(f)\mathbf{x}$. Since $\mathbf{w}^{(t)}\in {\cal X}$ and $\mathbf{x}\in {\cal X}$, we know that $\mathbf{w}^{(t+1)}\in {\cal X}$. This also shows that if we initialize $\mathbf{w} = \mathbf{w}_1 + \mathbf{w}_2$ that $\mathbf{w}_1 \in {\cal X}$ and $\mathbf{w}_2 \in {\cal X}^\perp$. $\mathbf{w}_2$ won't be changed during the gradient descent.}

It is also easy to see that with probability 1, $x_i$ will all be linearly independent, so that $dim({\cal X}) = n$, where $dim$ denotes the dimension of a subspace.  

We now define the notion of an $\epsilon$-adversarial point.  We say that $x$ is an $\epsilon$-adversarial point of $x_i$ if $\|x - x_i\| < \epsilon$, and $sign(y_i) \neq sign(f^*(x))$.  We can now prove the following theorem (for now, we give the theorem and proof informally)
\begin{theorem}
Given all assumptions mentioned above, for sufficiently large values of $d$ and $n$, with high probability, every point $x_i$ has an $\epsilon$-adversarial point.  
\end{theorem}
\begin{proof}
To see this, we first note that for any small value $\epsilon_0$, there is a sufficiently large $d$ such that with high probability, $x_i^Tx_j < \epsilon_0, \forall i,j, i \neq j$.  That is, all the $x_i, x_j$ are nearly orthogonal.

We now consider a $x_i$ with $y_i = 1$, and $x_j$ with $y_j = -1$.  Denote $v_{ij} = x_j - x_i$.  Then, since $f^*$ is linear, we have:
\[
\frac{\partial f^*}{\partial v_{ij}} = \frac{2}{\|v_{ij}\|} \approx \sqrt{2}
\]
\rb{Should be $\frac{\partial f^*}{\partial \hat v_{ij}}$.}
The right hand side is because, with high probability, we will also have $\|v_{ij}\|$ is nearly equal to $\sqrt{2}$.  We have:
\[
\|v_{ij}\|^2 = \|x_j - x_i\|^2 = \|x_i\|^2 + \|x_j\|^2 - 2x_j^Tx_i \approx 2
\]
because $x_i$ and $x_j$ are nearly orthogonal.

These partial derivatives are sufficient to allow us to compute the gradient of $f^*$ and its magnitude (note that the gradient of $f^* = w$.  So $w^T\hat{v}_{ij} \approx \sqrt{2}$, where $\hat{v}_{ij}$ is a unit vector parallel to $v_{ij}$).

For $j \neq k$, $v_{ij}$ and $v_{ik}$ are not orthogonal.  We have 
\[
v_{ij}^Tv_{ik} = (x_j - x_i)^T (x_k - x_i) \approx \|x_i\|^2 \approx 1
\]
because $x_i, x_j, x_k$ are all nearly orthogonal to each other. That is, $\hat{v}_{ij}^T\hat{v}_{ik} \approx \frac{1}{2}$, so the angle between the two vectors is $\frac{\pi}{3}$.

We can therefore write:
\[
\hat{v}_{ik} \approx \frac{1}{2}\hat{v}_{ij} + \sin{\frac{\pi}{3}}\hat{v}^\perp_{ik}
\]
where $\hat{v}^\perp_{ik}$ is a unit vector orthogonal to $v_{ij}$.
\rb{Shouldn't this be denoted $\hat{v}^\perp_{ij}$ then? Note also that $\sin(\pi/3)=\sqrt{3}/2.$}
This means:
\[
w^T\hat{v}_{ik} \approx \frac{1}{2}w^T\hat{v}_{ij} + \sin{\frac{\pi}{3}}w^T\hat{v}^\perp_{ik}
\]
and, since $w^T\hat{v}_{ij} \approx w^T \hat{v}_{ik} \approx \sqrt{2}$
we have:
\[
w^T \hat{v}^\perp_{ik} \approx \frac{\sqrt{2}}{2\sin{\frac{\pi}{3}}}
\]

We therefore also have 
\[
\frac{\partial f^*}{\partial \hat{v}^\perp_{ik}} \approx \frac{\sqrt{2}}{2\sin{\frac{\pi}{3}}}
\]

Finally, suppose we have some $x_i$ such that $y_i = 1$.  We select any $x_j$ such that $y_i = -1$.  Then we consider all $k \neq j$ for which $y_k = -1$.  The set of $\{x_j, x_k\} \forall k$ span a linear subspace, and the vectors $\hat{v}_{ij}, \hat{v}^\perp_{ik}$ form an orthonormal basis for this linear subspace.  For any direction orthogonal to this subspace, the partial derivative of $f^*$ is zero.  ({\em Maybe add some proof of this})
\sg{Proof by contradiction: suppose that for some direction $v^\prime$ that is orthogonal to this subspace, the gradient is not zero. WLOG, we assume $\frac{\partial f^*}{\partial v^\prime} < 0$. Since $f^*$ is linear, there exists some step size $\eta > 0$ that $f^*(x_i+\eta v^\prime) = -1$. This shows that vector $v^\prime$ is on the subspace which is contradicted by our assumption.}
So the gradient of $f^*$ is given by:
\[
\frac{\partial f^*}{\partial v_{ij}}, \frac{\partial f^*}{\partial \hat{v}^\perp_{ik}}
\]
Noting that about half the training points have a label of -1, we can conclude that:
\[
\| \nabla f^* \| \approx \sqrt{\frac{n}{2}} \frac{\sqrt{2}}{2\sin{\frac{\pi}{3}}} = \frac{\sqrt{n}}{2\sin{\frac{\pi}{3}}}
\]
\rb{Where is $\frac{\partial f^*}{\partial v_{ij}}\approx \sqrt{2}$?}

Because $f^*$ is linear, we can say that:
\[
f^*(x_i - \epsilon \nabla f^*) = 1 - \epsilon \| \nabla f^*\|
\]
when $y_i = 1$.  Therefore, for
\[
\epsilon > \frac{2\sin{\frac{\pi}{3}}}{\sqrt{n}}
\]
$sign(f^*(x_i - \epsilon  \nabla f^*) = -1$ and $x_i - \epsilon  \nabla f^*$ is an adversarial example.  By choosing $n$ sufficiently large, we can create an $\epsilon$-adversarial example.
\end{proof}

This results shows that there are adversarial examples near the training data.  Note that if we have test data that is also correctly labeled by $f^*$, exactly the same reasoning shows that there will also be adversarial examples near the test data.

\subsection{Extension to general functions}

Of course, if $f^*$ is a completely general function, we cannot say anything about its gradient, or the existence of adversarial examples.  However, to gain some intuition, we consider a special case.  Suppose, for all $x_i$ with $y_i = 1$ and for all $x_j$ with $y_j = -1$ we have:
\[
\frac{\partial f^*}{\partial v_{ij}} \ge \frac{2}{\|v_{ij}\|} \approx \sqrt{2}
\]
Then the theorem from the previous section still holds.

What does this assumption say?  One way to think about it to consider the value of $f^*$ along the line segment from $x_i$ to $x_j$.  The function must decrease from 1 to -1 along this line segment.  This assumption just says that the rate of decrease at $x_i$ is at least as large as the average rate of decrease along the whole line segment.

\subsection{Extensions to $d < n$}

{\em Basically, if $d < n$, as is true in real cases, we can still apply the theorem.  We just need to determine how close to orthonormal the data is.  We build up a basis one element at a time.  The second $x$ is almost orthonormal to the first.  Then the third is a little less orthonormal to the first two.  This reduces the effect slightly.  Then we keep doing that.  If the $x$ are Gasussian distributed, it should be possible to quantify this.}

\subsection{Regularization}


\begin{figure}[t]
    \centering
    \includegraphics[height=5.0cm]{figures/LinearInterpolation.png}
    \includegraphics[height=5.0cm]{figures/RobustInterpolation.png}
    \includegraphics[height=5.0cm]{figures/SmoothTraining.png}
    
    \caption{\small Different ways of interpolating between points.}
    \label{fig:interpolation}
\end{figure}

These theorems may give us some insight into the effect of regularization on adversarial examples.  We consider regularization by limiting the Lipschitz constant of the interpolating function, or by limiting the curvature (eg., via the largest eigenvalue of the Hessian).  We also consider global and local regularization.  Global regularizes the entire function, eg., by limiting the Lipschitz constant of the function.  Local regularizes the function only at the training data, eg., by penalizing large curvature at these points.  

Refer to Figure \ref{fig:interpolation}, which shows four points in a 1D example.  The top illustrates a linear interpolation between $x_2$ for which $y_2 = -1$ and $x_3$, for which $y_3 = 1$.  We have seen before that this linear interpolation can lead to large gradients that give rise to adversarial examples.  However, if we define an interpolating function as one which exactly matches the training labels, then we note that this interpolating function is the one with minimum Lipschitz constant.  On the other hand, the middle graph shows the most robust interpolating function.  This, however, has a very high Lipschitz constant.  Therefore, Lipschitz regularization may actually lead to a function that is less robust.  {\em This argument is pretty half-baked, since it only applies to 1D.  Things would be much more complicated in higher dimensions. }

The bottom graph illustrates what could happen if we locally regularize the interpolating function, requiring it to have low gradient and low Hessian eigenvalues at the location of the training data.  The function will be flat near the training data, producing a modest amount of robustness.  But it can then interpolate linearly, producing adversarial examples in the region of linear interpolation.  We conjecture that this bottom graph relects what can happen with adversarial training.  The interpolating function is flattened near the adversarial example, but can then interpolate in ways that produce new adversarial examples.


\subsection{Experiments}

It's not clear how to use experiments to determine if this simple theory is relevant to real networks.  For one thing, in real problems, we do not have $n << d$.  The theory should perhaps be extended to handle the case of $d < n$.  But we could check a couple of things.  We might do this for a simple case, like a network with a single hidden layer trained on MNist, or a more complicated case, like a real network trained on ImageNet.

\begin{itemize}
    \item Is the gradient magnitude actually large at the location of training examples?
    \item Do we actually find:
    \[
\frac{\partial f^*}{\partial v_{ij}} \ge \frac{2}{\|v_{ij}\|} \approx \sqrt{2}
\]
(more or less) in real data?  In looking at this, it might also make sense to check the partial derivative {\em near} the training point, but not exactly at it.  That is, look the partial derivative at $x_i + \epsilon v_{ij}$, for some $\epsilon$.
\end{itemize}


